Preventing Rowhammer Exploits via Low-Cost Domain-Aware Memory Allocation

Rowhammer is a hardware security vulnerability at the heart of every system with modern DRAM-based memory. Despite its discovery a decade ago, comprehensive defenses remain elusive, while the probability of successful attacks grows with DRAM density. Hardware-based defenses have been ineffective, due to considerable cost, delays in commercial adoption, and attackers' repeated ability to circumvent them. Meanwhile, more flexible software-based solutions either incur substantial performance and memory capacity overheads, or offer limited forms of protection. Citadel is a new memory allocator design that prevents Rowhammer-initiated security exploits by addressing the vulnerability's root cause: physical adjacency of DRAM rows. Citadel enables creation of flexible security domains and isolates different domains in physically disjoint memory regions, guaranteeing security by design. On a server system, Citadel supports thousands of security domains at a modest 7.4% average memory overhead and no performance loss. In contrast, recent domain isolation schemes fail to support many workload scenarios due to excessive overheads, and incur 4--6x higher overheads for supported scenarios. As a software solution, Citadel offers readily deployable Rowhammer-aware isolation on legacy, current, and future systems.

==> acks.tex <==
Moin, Sibi
Ada?


==> cmds.tex <==

\newcommand{\red}[1]{\noindent{\color{red}{#1}}}

\newcommand\ad[1]{\noindent{\color{red} {\bf \fbox{Alex:}}{\bf \it#1}}}
\newcommand\as[1]{\noindent{\color{green} {\bf \fbox{Anish:}}{\bf \it#1}}}
\newcommand\ww[1]{\noindent{\color{blue} {\bf \fbox{Walter:}}{\bf \it#1}}}
\newcommand\revision[1]{{\color{black} {#1}}}
\newcommand\usenix[1]{{\color{black} {#1}}}

\newcommand\mytodo[1]{\noindent{\color{orange} {\bf \fbox{TODO}}{\bf \it#1}}}

\newcommand\TheName{Citadel\xspace}

\newcommand\aegisAvgStranding{{5.8\%}\xspace}
\newcommand\aegisAvgLoss{{1.6\%}\xspace}
\newcommand\aegisAvgOverhead{{7.4\%}\xspace}
\newcommand\silozAvgOverhead{{33\%}\xspace}


\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.5pt, fill=white, text=black] (char) {#1};}}

\Crefname{figure}{Fig.}{Figs.}
\crefname{figure}{Fig.}{Figs.}
\crefformat{section}{#2§#1#3}
\crefformat{subsection}{#2\S#1#3}
\crefformat{subsubsection}{#2\S#1#3}

